The Problem of Infra-marginality in Outcome Tests for Discrimination

Outcome tests are a popular method for detecting bias in lending, hiring, and policing decisions. These tests operate by comparing the success rate of decisions across groups. For example, if loans made to minority applicants are observed to be repaid more often than loans made to whites, it suggests that only exceptionally qualified minorities are granted loans, indicating discrimination. Outcome tests, however, are known to suffer from the problem of infra-marginality: even absent discrimination, the repayment rates for minority and white loan recipients might differ if the two groups have different risk distributions. Thus, at least in theory, outcome tests can fail to accurately detect discrimination. We develop a new statistical test of discrimination---the threshold test---that mitigates the problem of infra-marginality by jointly estimating decision thresholds and risk distributions via a hierarchical Bayesian latent variable model. Applying our test to a dataset of 4.5 million police stops in North Carolina, we find that the problem of infra-marginality is more than a theoretical possibility, and can cause the outcome test to yield misleading results in practice.

==> tab2.tex <==
% latex table generated in R 3.2.3 by xtable 1.8-0 package
% Thu Jun  9 21:03:25 2016
\begin{table}[t]
\centering
\makebox[\textwidth][c]{
\begin{tabular}{lrr}
  \toprule
Driver race & Search threshold & 95\% credible interval \\ 
  \midrule
White & 15\% & (14\%, 16\%) \\ 
  Black & 7\% & (3\%, 10\%) \\ 
  Hispanic & 6\% & (5\%, 8\%) \\ 
  Asian & 13\% & (11\%, 16\%) \\ 
   \bottomrule
\end{tabular}}
\caption{\emph{Inferred search thresholds for stops conducted by the 100 largest police departments in North Carolina. For each race group, we report the average threshold across departments, weighting by the number of stops conducted by the department. We find black and Hispanic drivers face lower search thresholds than white and Asian drivers.}} 
\label{tab:threshold_results}
\end{table}

